Self-Consistent Reasoning-based Aspect-Sentiment Quad Prediction with Extract-Then-Assign Strategy

In the task of aspect sentiment quad prediction (ASQP), generative methods for predicting sentiment quads have shown promising results. However, they still suffer from imprecise predictions and limited interpretability, caused by data scarcity and inadequate modeling of the quadruplet composition process. In this paper, we propose Self-Consistent Reasoning-based Aspect-sentiment quadruple Prediction (SCRAP), optimizing its model to generate reasonings and the corresponding sentiment quadruplets in sequence. SCRAP adopts the Extract-Then-Assign reasoning strategy, which closely mimics human cognition. In the end, SCRAP significantly improves the model's ability to handle complex reasoning tasks and correctly predict quadruplets through consistency voting, resulting in enhanced interpretability and accuracy in ASQP.

==> 081fewshot.tex <==
\onecolumn\
\begin{mdframed}
\captionof{table}{LLM few shot prompt}
\label{tab:few_shot_prompt_old}
\noindent 
\newline
\small I am performing the ASQP task, which is the Subtask of ABSA. From now on, if I give you a sentence and a quadruplet, create a Reasoning for it. 

\noindent
\newline
\small When creating, create to satisfy all of the following conditions: 
\newline

When proceeding with inference, extract the aspect term and the option term first and infer the aspect category and sentimental polarity based on them. When extracting aspect term and option term, an aspect category is judged by a combination of aspect term and opinion term, and sentimental polarity is judged by comprehensively considering everything. And don't mention each element first, explain the reason first, and then create a rationale that mentions the element. At this time, do not number each element, but configure it to naturally lead to one paragraph. But if there are more than two quadruplets, please organize the description for each quadruplet. And please create a detailed description of each element in the composition of rationale. From now on, I'll give you sentences and quadruplet sets as input.

\noindent
\newline
\small Here are possible aspect category set: ['food prices', 'food style\_options', 'service general', 'drinks prices', 'ambience general', 'drinks quality', 'location general', 'restaurant prices', 'restaurant general', 'drinks style\_options', 'food general', 'restaurant miscellaneous', 'food quality'].

\noindent
\newline
\small Here are possible sentiment polarity set: ['positive','negative','neutral'].

\noindent
\newline
\small Sentence: The fried dumplings are GREAT !\#\#\#\#[['fried dumplings', 'food quality', 'positive', 'GREAT']]
\noindent
\newline    
\small Reasoning : In this sentence, the aspect term is ‘fried dumplings’ and the opinion term for this aspect term is ‘GREAT’. Since the aspect term is ‘fried dumplings’ and the opinion about the aspect term is ‘GREAT’, the aspect category can be inferred as ‘food quality’ for this aspect term. Lastly, the aspect term ‘fried dumplings’ is evaluated as a opinion of ‘GREAT’. When it comes to food, the opinion 'GREAT' suggests that the food is delicious, which is evaluated as a positive sentiment.

\noindent
\newline
\small Sentence: It's one of our favorite places to eat in NY.\#\#\#\#[['NULL', 'restaurant general', 'positive', 'favorite']]
\noindent
\newline
\small Reasoning : In this sentence, there is no specific aspect term mentioned explicitly. So the aspect term is ‘NULL’ and the opinion term for this aspect term is ‘favorite’. The aspect category could be inferred as 'restaurant general' as the speaker is expressing a general sentiment about the restaurant rather than a specific feature or component. Lastly, by referring to the restaurant as a 'favorite', the speaker implies a positive sentiment polarity.

\noindent
\newline
\small Sentence: It is very overpriced and not very tasty .\#\#\#\#[['NULL', 'food quality', 'negative', 'not very tasty'], ['NULL', 'food prices', 'negative', 'overpriced']]
\noindent
\newline
\small Reasoning : In the sentence, there are two different evaluations made but none of them explicitly mentions the specific aspect term. So, for both evaluations, the aspect term is 'NULL'. For the first quadruplet, the opinion term is 'not very tasty'. This is a negative evaluation of the food quality, hence 'food quality' can be inferred as the aspect category and the sentiment polarity is negative. In the second quadruplet, the opinion term is 'overpriced'. This term is often used to describe something that is too expensive or not worth the price. Therefore, the aspect category can be inferred as 'food prices' and since the speaker is expressing a negative sentiment about the price, the sentiment polarity is negative.

\noindent
\newline
\small Sentence: The service was friendly and the atmosphere was casual .\#\#\#\#[['service', 'service general', 'positive', 'friendly'], ['atmosphere', 'ambience general', 'neutral', 'casual']]
\noindent
\newline
\small Reasoning : The sentence discusses two aspects - 'service' and 'atmosphere'. For the first quadruplet, the aspect term is 'service' and the opinion term is 'friendly'. This is a positive evaluation of the service provided by the restaurant, hence 'service general' can be inferred as the aspect category and the sentiment polarity is positive. In the second quadruplet, the aspect term is 'atmosphere' and the opinion term is 'casual'. This term is used to describe the general ambience of the restaurant. Therefore, the aspect category can be inferred as 'ambience general'. As the term 'casual' is neutral and doesn't indicate any positive or negative sentiment, the sentiment polarity is neutral.
    
\noindent
\newline
\small Sentence: Rude service , medicore food ... there are tons of restaurants in NY ... stay away from this one\#\#\#\#[['service', 'service general', 'negative', 'Rude'], ['food', 'food quality', 'neutral', 'medicore'], ['NULL', 'restaurant general', 'negative', 'stay away']]
\noindent
\newline
\small Reasoning : The sentence discusses three aspects - 'service', 'food', and the general experience at the restaurant (NULL). For the first quadruplet, the aspect term is 'service' and the opinion term is 'Rude'. This is a negative assessment of the service provided by the restaurant, hence 'service general' can be inferred as the aspect category and the sentiment polarity is negative. In the second quadruplet, the aspect term is 'food' and the opinion term is 'medicore'. This term is used to describe the quality of the food at the restaurant. Therefore, the aspect category can be inferred as 'food quality'. As the term 'medicore' is neutral and doesn't indicate any positive or negative sentiment, the sentiment polarity is neutral. In the third quadruplet, there is no specific aspect term mentioned, so the aspect term is 'NULL'. The opinion term is 'stay away'. This is a negative sentiment about the restaurant in general, hence 'restaurant general' can be inferred as the aspect category and the sentiment polarity is negative.
% \caption{LLM few shot prompt}\label{tab:few_shot_prompt}
% \captionof{table}{LLM few shot prompt}\label{tab:few_shot_prompt}
\end{mdframed}


\begin{mdframed}
\captionof{table}{Input-Target example}
\label{tab:target_example}
\small Input: we have gone for dinner only a few times but the same great quality and service is given .

\noindent
\newline
\small Target : in this sentence, the speaker mentions their experience of going for dinner a few times. they highlight the consistent great quality and service they have received. for the first quadruplet, the aspect term is 'service' and the opinion term is 'great'. this indicates a positive evaluation of the service provided by the restaurant. therefore, the aspect category can be inferred as 'service general' and the sentiment polarity is positive. for the second quadruplet, the aspect term is 'dinner' and the opinion term is 'great quality'. this implies a positive assessment of the quality of the food during dinner. hence, the aspect category can be inferred as 'food quality' and the sentiment polarity is positive.the speaker's statement overall conveys their positive experience, emphasizing the consistent great quality and service they have received during their visits for dinner. therefore, the quadruplets are: [SP] positive [AT] dinner [OT] great quality [AC] food quality [SSEP] [SP] positive [AT] service [OT] great [AC] service general
\end{mdframed}
